Hypo-elasticity, Cauchy-elasticity, corotational stability and monotonicity in the logarithmic strain

We combine the rate-formulation for the objective, corotational Zaremba-Jaumann rate \begin{align} \frac{{\rm D}^{\rm ZJ}}{{\rm D} t} [\sigma] = \mathbb{H}^{\rm ZJ}(\sigma).D, \qquad D = {\rm sym} {\rm D} v\,, \end{align} operating on the Cauchy stress $\sigma$, the Eulerian strain rate $D$ and the spatial velocity $v$ with the novel \enquote{corotational stability postulate} (CSP)\begin{equation} \Bigl\langle \frac{{\rm D}^{\rm ZJ}}{{\rm D} t}[\sigma], D \Bigr\rangle > 0 \qquad \forall \, D\in{\rm Sym}(3)\setminus\{0\} \end{equation} to show that for a given isotropic Cauchy-elastic constitutive law $B \mapsto \sigma(B)$ in terms of the left Cauchy-Green tensor $B = F F^T$, the induced fourth-order tangent stiffness tensor $\mathbb{H}^{\rm ZJ}(\sigma)$ is positive definite if and only if for $\widehat{\sigma}(\log B):=\sigma(B)$, the strong monotonicity condition (TSTS-M$^{++}$) in the logarithmic strain is satisfied. Thus (CSP) implies (TSTS-M^{++}) and vice-versa, and both imply the invertibility of the hypo-elastic material law between the stress and strain rates given by the tensor $\mathbb{H}^{\rm ZJ}(\sigma)$. The same characterization remains true for the corotational Green-Naghdi rate as well as the corotational logarithmic rate, conferring the corotational stability postulate (CSP) together with the monotonicity in the logarithmic strain tensor (TSTS-M^{++}) a far reaching generality. It is conjectured that this characterization of (CSP) holds for a large class of reasonable corotational rates. The result for the logarithmic rate is based on a novel chain rule for corotational derivatives of isotropic tensor functions.

==> figures/diagram.tex <==
%
\begin{tikzpicture}
\node (A) at (0,0) {%
	$\displaystyle
	\left.
		\begin{array}{llc}
		&\Bigg\{&
			\begin{array}{c}
			\textbf{corotational stability postulate (CSP)} \\ 
			\textbf{for the Cauchy stress $\sigma$} \\
			\langle \frac{\DD^{\ZJ}}{\DD t}[\sigma], D \rangle = \langle \H^{\ZJ}(\sigma).D,D \rangle > 0 \\
			\end{array}
		\\
		\iff \quad &\Bigg\{&
			\begin{array}{c}
			\textbf{TSTS-M$^{++}$}: \\
			\sym \DD_{\log B} \widehat \sigma(\log B) \in \Sym^{++}_4(6) \\
			\implies \quad \langle \widehat \sigma(\log V_1) - \widehat \sigma(\log V_2), \log V_1 - \log V_2 \rangle > 0
			\end{array}
		\end{array}
	\right\}
	$
};
\node at (5.88,0) {%
$\displaystyle
	\notiff
	$
};
\node (B) at (10.29,0) {%
$\displaystyle
	\left\{
		\begin{array}{l}
		\textbf{Legendre-Hadamard ellipticity}: \\
		\DD_F^2 \WW(F). (\xi \otimes \eta, \xi \otimes \eta) \ge c^+ \, |\xi|^2 \cdot |\eta|^2 \\
		\langle S_1(F + \xi \otimes \eta) - S_1(F), \xi \otimes \eta \rangle \ge c^+ \, |\xi|^2 \, |\eta|^2
		\end{array} \right.
		\vphantom{
			\begin{array}{llc}
			&\Bigg\{&
				\begin{array}{c}
				\textbf{corotational stability postulate (CSP)} \\ 
				\textbf{for the Cauchy stress $\sigma$} \\
				\langle \frac{\DD^{\ZJ}}{\DD t}[\sigma], D \rangle = \langle \H^{\ZJ}(\sigma).D,D \rangle > 0 \\
				\end{array}
			\\
			\iff \quad &\Bigg\{&
				\begin{array}{c}
				\textbf{TSTS-M$^{++}$}: \\
				\sym \DD_{\log B} \widehat \sigma(\log B) \in \Sym^{++}_4(6) \\
				\implies \quad \langle \widehat \sigma(\log V_1) - \widehat \sigma(\log V_2), \log V_1 - \log V_2 \rangle > 0
				\end{array}
			\end{array}
		}
	$
};
\node (C) at (-.98,-3.43) {%
	$\displaystyle
	\textnormal{BE}: \quad (\sigma_i - \sigma_j) \, (\lambda_i - \lambda_j) \ge 0
	\vphantom{
		\textnormal{TE\footnotemark}: \quad \frac{\partial \sigma_i(\lambda_1, \lambda_2, \lambda_3)}{\partial \lambda_i} \ge 0 \quad \iff \quad \frac{\partial \widehat \sigma_i(\log \lambda_1, \log \lambda_2, \log \lambda_3)}{\partial \log \lambda_i} \ge 0
	}
	$
};
\node (D) at (8.33,-3.43) {%
	$\displaystyle
	\textnormal{TE\footnotemark}: \quad \frac{\partial \sigma_i(\lambda_1, \lambda_2, \lambda_3)}{\partial \lambda_i} \ge 0 \quad \iff \quad \frac{\partial \widehat \sigma_i(\log \lambda_1, \log \lambda_2, \log \lambda_3)}{\partial \log \lambda_i} \ge 0
	$
};

\coordinate (X) at ($(B.south west)!.5!(B.south)$);
\draw[-implies,double equal sign distance] (A) -- (C.north-|A);
\draw[-implies,double equal sign distance] (A.south) -- ($(D.north west)!.5!(D.north)$);
\draw[-implies,double equal sign distance] (X) -- (C.north east);
\draw[-implies,double equal sign distance] (X) -- (D.north-|X);
\end{tikzpicture}
%
